A Practical Sparse Approximation for Real Time Recurrent Learning

Current methods for training recurrent neural networks are based on backpropagation through time, which requires storing a complete history of network states, and prohibits updating the weights `online' (after every timestep). Real Time Recurrent Learning (RTRL) eliminates the need for history storage and allows for online weight updates, but does so at the expense of computational costs that are quartic in the state size. This renders RTRL training intractable for all but the smallest networks, even ones that are made highly sparse. We introduce the Sparse n-step Approximation (SnAp) to the RTRL influence matrix, which only keeps entries that are nonzero within n steps of the recurrent core. SnAp with n=1 is no more expensive than backpropagation, and we find that it substantially outperforms other RTRL approximations with comparable costs such as Unbiased Online Recurrent Optimization. For highly sparse networks, SnAp with n=2 remains tractable and can outperform backpropagation through time in terms of learning speed when updates are done online. SnAp becomes equivalent to RTRL when n is large.

==> Sparse RTRL Arxiv/costs_figure.tex <==
\begin{figure}
\begin{floatrow}
\ffigbox{
\includegraphics[width=0.48\textwidth]{RTRL_Diagrams_2.png}
}{
\caption{Depiction of RTRL, RTRL with sparsity and SnAp.
White indicates zeros. (a) $I_t + D_tJ_{t-1}$ (b) $I_t + D_tJ_{t-1}$ when $W$ is sparse (c) $\tilde{I}_t + D_t\tilde{J}_{t-1}$ (d) SnAp-2 (e) SnAp-1. Rose colored squares are non-zero in $D_t$ but not used in updating $J_t$.}
\label{fig:costs_figure}
}
\capbtabbox{

\begin{tabular}{l|l|l}
\toprule
Method & memory & time per step \\ 
\midrule
BPTT & $Tk + p$ & $k^2 + p$ \\
UORO & $k + p$ & $k^2 + p$ \\
RTRL & $k + kp$ & $k^2 + k^2p$ \\
\midrule
Sparse BPTT & $Tk + dp$ & $d (k^2 + p)$ \\
Sparse RTRL & $k + dkp$ & $d(k^2 + dk^2p)$ \\
SnAp-1 & $k + dp$ & $d(k^2 + p)$ \\
SnAp-2 & $k + d^2kp$ & $d(k^2 + d^2k^2p)$ \\
\bottomrule
\end{tabular}
}{
\caption{Computational costs of gradient calculation methods for dense and sparse RNNs. Below $T$ refers to the sequence length, $k$ the number of hidden units, $p$ the number of recurrent parameters, $s$ the level of sparsity, and $d = 1 - s$.}
\label{costs_table}
}
\end{floatrow}
\end{figure}

==> Sparse RTRL Arxiv/flops_table.tex <==
\setlength{\tabcolsep}{.4em}
\renewcommand\arraystretch{.7}
\begin{table*}[h]
\caption{Empirical computational costs of SnAp, determined by the sparsity level in the Jacobians. The ``X vs BPTT'' rows express the FLOPS requirements of X as a multiple of BPTT training FLOPs. The ``SnAp-2 vs RTRL'' row shows the FLOPS requirements of SnAp-2 as a multiple of those required by optimized Sparse RTRL (section \ref{sparse_optimizations}). Lower is better for all of these entries.}
\label{flops_table}
\begin{center}
\begin{tabular}{c||c|c|c||c|c|c||c|c|c}
\toprule
Architecture & \multicolumn{3}{c||}{Vanilla} & \multicolumn{3}{c||}{GRU} & \multicolumn{3}{c}{LSTM} \\
\midrule
Number of Units & 128 & 256 & 512 & 128 & 256 & 512 & 128 & 256 & 512 \\
Param. Sparsity & 75.0\% & 93.8\% & 98.4\% & 75\% & 93.8\% & 98.4\% & 75.0\% & 93.8\% & 98.4\% \\
SnAp-2 J Sparsity & 83.0\% & 95.6\% & 98.9\% & 70.9\% & 91.1\% & 97.8\% & 38.5\% & 79.9\% & 95.1\%  \\
SnAp-3 J Sparsity & 33.3\% & 59.2\% & 92.8\% & 50.0\% & 52.5\% & 71.6\% & 2.4\% & 5.9\% & 38.7\%  \\
SnAp-1 vs BPTT & 1x & 1x & 1x & 1x & 1x & 1x & 2x & 2x & 2x \\
SnAp-2 vs BPTT & 349x & 90.4x & 22.1x & 597x & 183x & 44.8x & 2518x & 824.8x & 200.1x \\
SnAp-3 vs BPTT & 1365x & 835.8x & 147.5x & 1024x & 972x & 582x & 3996x & 3855x & 2513x \\
SnAp-2 vs RTRL & 0.17x & 0.044x & 0.011x & 0.291x & 0.089x &  0.022x &  0.615x & 0.201x & 0.049x \\
\bottomrule
\end{tabular}
\vspace{-0.5em}
\end{center}
\end{table*}

==> Sparse RTRL Arxiv/pruning_figure.tex <==
\begin{figure}
\begin{floatrow}
\ffigbox{
\includegraphics[width=0.9\linewidth]{paper_pruning_plot.png}
}{
\caption{BPC vs Sparsity for Constant Parameter Count. Shows the same results as Table \ref{pruning_table}. The biggest, sparsest GRU performs better than a dense network with 6.25x as many (nonzero) parameters.}
\label{fig:pruning_figure}
}
\capbtabbox{
\begin{tabular}{l||l|l|l}
\toprule
units & bpc & $\theta$ sparsity & $|\theta|$ \\
\midrule
base & 1.55 & 0\% & 1x \\
2x & 1.48 & 75\% & 1x \\
4x & 1.43 & 93.75\% & 1x \\
8x & 1.42 & 98.4\% & 1x \\
16x & 1.40 & 99.6\% & 1x \\
\bf{32x} & \bf{1.38} & \bf{99.9}\% & \bf{1x} \\
2.5x & 1.39 & 0\% & 6.25x \\
\bottomrule
\end{tabular}
}{
\caption{Final performance of sparse WikiText103 language modeling GRU networks trained with progressive pruning. Each row represents a single training run. The `bpc' column gives the validation set negative log-likelihood in units of bits per character. The $|\theta|$ column gives the number of parameters in the network as a multiple of the `base' 128-unit model.}
\label{pruning_table}
}
\end{floatrow}
\end{figure}
